Comparative Analysis of Non-thermal Emissions and Study of Electron Transport in a Solar Flare

We study the non-thermal emissions in a solar flare occurring on 2003 May 29 by using RHESSI hard X-ray (HXR) and Nobeyama microwave observations. This flare shows several typical behaviors of the HXR and microwave emissions: time delay of microwave peaks relative to HXR peaks, loop-top microwave and footpoint HXR sources, and a harder electron energy distribution inferred from the microwave spectrum than from the HXR spectrum. In addition, we found that the time profile of the spectral index of the higher-energy ($\gsim 100$ keV) HXRs is similar to that of the microwaves, and is delayed from that of the lower-energy ($\lsim 100$ keV) HXRs. We interpret these observations in terms of an electron transport model called {\TPP}. We numerically solved the spatially-homogeneous {\FP} equation to determine electron evolution in energy and pitch-angle space. By comparing the behaviors of the HXR and microwave emissions predicted by the model with the observations, we discuss the pitch-angle distribution of the electrons injected into the flare site. We found that the observed spectral variations can qualitatively be explained if the injected electrons have a pitch-angle distribution concentrated perpendicular to the magnetic field lines rather than isotropic distribution.

==> response <==

Dear Timothy S. Bastian,

     Re: ApJ Submission MS# 71652

Thank you very much for sending us the referee's report on our paper,

     "Comparative Analysis of Non-Thermal Emissions and Study of Electron Transport in a Solar Flare", by Minoshima et al.

We have revised the manuscript.
Here, I will send you the revised version through the web.
The followings are our answers to the referee's reports.

-------------------------------------------------------

I am very happy that the referee has recommended our paper for publication in ApJ.
I deeply appreciate that you read carefully, well understand and kindly correct our paper and encourage me throughout the revision.
Without your help, I would never achieve such an improvement of our paper.

The followings are our answer to the referee's comments

-----------------------------
-1. Page 2, Bastian (1999) may not the best reference. Usually Ramaty (1969) and Brown (1971) are used to introduce gyrosynchrotron and bremsstrahlung mechanisms, respectively. If authors intended to focus on energies of radiating electrons, Nitta & Kosugi (1986) may be more appropriate.


 I changed the statement as follows:

Because HXRs are emitted primarily by electrons with energy below several hundred keV via {\bremss} radiation, whereas microwaves are emitted by electrons above several hundred keV via gyrosynchrotron (Bastian 1999)
-> Because HXRs below $\sim 100$ keV are emitted primarily by electrons with energy below several hundred keV via {\bremss} radiation (Brown 1971), whereas microwaves above $\sim 10$ GHz are emitted by electrons above several hundred keV via gyrosynchrotron (Ramaty 1969; Bastian 1999)
   


-2. The 6th paragraph of Sect.1 (page 3) is quite problematic. I understand that authors want to illustrate importance of imaging with examples. But the paper citation did not work in that way.  First, Silva et al. (1997) presented (emphasized) an imaging observation at both radio and X-rays to show spatial coincidence of both sources was not assumed. Silva et al. (2000) is indeed based on non-imaging results to speculate on the source structure and pitch angle diffusion, and this is the right paper to cite. However, what they described is rather close to weak diffusion as opposed to strongEdiffusion. Also note that under TPP model, radio and HXR sources need not spatially coincide with each other. Authors interpretations given there sound like accusing those works with unfair incorrect judgments. I think it can be modified to the following form or similar:


 I apologize that I might unintentionally criticize the works of Silva et al. with unfair way. The 6th and 7th paragraphs of Sec. 1 is combined and is changed as follows:

There have been many observations that can be explained in terms of the TPP model. Yokoyama et al (200) reported ...... the microwave observation. Silva et al. (2000) pointed out that the discrepancy of the energy distribution between the HXR and microwave emitting electrons found in their study could be explained by the TPP model. In their study, there was no imaging observation to confirm their suggestion. If the HXR and microwave sources do not coincide spatially, the discrepancy of the energy distribution between the HXR and microwave emitting electrons can be explained by the different spatial distribution between the HXR and microwave emitting electrons as a result of the TPP model. Imaging as well as spectral data at both HXR and microwave wavelengths are essential to confirm the role of TPP on the parent electrons




-3. One thing I found odd with this paper is that authors repeatedly say the microwave spectral index is quite harder than the HXR spectral indices, which indicates that the inferred energy distribution of the microwave emitting electrons is harder than that of the HXR emitting ones.EI don't understand why authors keep saying so. As I commented earlier, one cannot directly judge this simply based on comparison of microwave spectral index with HXR spectral index because they are different radiation mechanisms.  Maybe, authors misuse "indicate" for "imply"? Otherwise, authors assume that readers have a conversion table for radio/HXR spectral index to electron power-law index? In any case, I suggest authors clarify this statement, at least, in the first place of the paper: on page 7, lines 8E1 can change to:


 The reason why I use such expression (microwave is harder than HXR) is that I would describe the difference of HXR and microwave spectral indices (eq. 18) and explain it from the different (energy and spatial) distribution of electrons.
 I understand what the referee pointed out, and realize that the direct comparison of the microwave and HXR spectral indices is physically no mean.
 Then I changed several related expressions as follows:

In Page 7:
The microwave spectral index is quite harder than the HXR spectral indices, which indicates that the inferred energy distribution of the microwave emitting electrons is harder than that of the HXR emitting ones.
-> The values of the microwave spectral index are quite smaller than those of the HXR spectral indices. This implies that the inferred energy distribution of the microwave emitting electrons is harder than that of the HXR emitting ones. We will carry out a spectral analysis in {\S} \ref{sec4} to confirm whether the energy distribution of the microwave emitting electrons is actually harder than that of the HXR emitting ones.

In Page 15:
The calculated microwave spectral indices are harder by $\sim 1.5-2$ than those of the HXRs in both the pancake and isotropic cases.
-> The values of the microwave spectral indices are smaller by $\sim 1.5-2$ than those of the HXR spectral indices in both the pancake and isotropic cases.

In Page 17:
The microwave spectral indices are harder by $\sim 2$ than that of the HXRs, indicating that the energy distribution of the microwave emitting electrons is harder than that of the HXR emitting ones.
-> The spectra of microwaves and HXRs imply that the microwave emitting electrons have a harder energy distribution than the HXR emitting ones.



-4. In the last paragraph on page 12, I think it better to change: 
no difference -> no much difference
independent -> almost independent
-5. Likewise, in the last paragraph on page 15:
no difference -> no much difference

 I followed your advice. 



-6. below equation (16), it is necessary to insert:

 I added the following sentence below eq. (16)

 Although this relationship is derived under the assumption that the parent electrons have an isotropic pitch-angle distribution, we use it for a rough estimate of the microwave spectral index from electrons with an arbitrary pitch-angle distribution. For HXRs, we can use equation (13) that shows the energy distribution of the precipitating electron flux, $F_{\mu}(E) \propto E^{-(\Delta-x)}$.



-7. The very first sentence in Section 4.3 does not read well. It can be changed to: 

 I changed the expression following your advice:

we discuss differences of the calculation results attributed to the difference of the pitch-angle distribution of the injection, without showing calculations with different values of ...
-> we have utilized the model electron distributions calculated for only two different types of the injection pitch-angle distribution (pancake and isotropic) with nominal values of parameters: ...



8. page 18, line 5-7 can change to:

I also changed the expression following your advice:

 Further, we discussed that a pancake pitch-angle distribution for the injected electrons rather than an isotropic distribution is reasonable to qualitatively explain the temporal variation of $\gammat{H}{obs}$.
-> We further found that a pancake pitch-angle distribution for the injected electrons rather than an isotropic distribution is more adequate to qualitatively explain the temporal variation of $\gammat{H}{obs}$.

-------------------------------------------------------

